Integration of Federated Learning and Blockchain in Healthcare: A Tutorial

Wearable devices and medical sensors revolutionize health monitoring, raising concerns about data privacy in ML for healthcare. This tutorial explores FL and BC integration, offering a secure and privacy-preserving approach to healthcare analytics. FL enables decentralized model training on local devices at healthcare institutions, keeping patient data localized. This facilitates collaborative model development without compromising privacy. However, FL introduces vulnerabilities. BC, with its tamper-proof ledger and smart contracts, provides a robust framework for secure collaborative learning in FL. After presenting a taxonomy for the various types of data used in ML in medical applications, and a concise review of ML techniques for healthcare use cases, this tutorial explores three integration architectures for balancing decentralization, scalability, and reliability in healthcare data. Furthermore, it investigates how BCFL enhances data security and collaboration in disease prediction, medical image analysis, patient monitoring, and drug discovery. By providing a tutorial on FL, blockchain, and their integration, along with a review of BCFL applications, this paper serves as a valuable resource for researchers and practitioners seeking to leverage these technologies for secure and privacy-preserving healthcare ML. It aims to accelerate advancements in secure and collaborative healthcare analytics, ultimately improving patient outcomes.

==> abreviation.tex <==
\acro{FL}{Federated Learning}
\acro{BCFL}{Blockchain-based Federated Learning}
\acro{HFL}{Horizontal Federated Learning}
\acro{VFL}{Vertical Federated Learning}
\acro{SMPC}{Secure Multi-Party Computation}
\acro{FTL}{Federated Transfer Learning}
\acro{HIPAA}{Health Insurance Portability and Accountability Act}
\acro{GDPR}{General Data Protection Regulation}
\acro{AI}{Artificial Intelligence}
\acro{BC}{Blockchain}
\acro{EHRs}{Electronic Health Records}
\acro{CT}{Computed Tomography}
\acro{MRI}{Magnetic Resonance Imaging}
\acro{PET}{Positron Emission Tomography}
\acro{DICOM}{Digital Imaging and Communications in Medicine}
\acro{CAD}{Computer-Aided Detection}
\acro{SNPs}{Single Nucleotide Polymorphisms}
\acro{CNVs}{Copy Number Variations}
\acro{RNA-seq}{RNA Sequencing}
\acro{ECG}{Electrocardiogram}
\acro{EMG}{Electromyography}
\acro{CGM}{Continuous Glucose Monitoring}
\acro{PGD}{Patient-Generated Data}
\acro{NLP}{Natural Language Processing}
\acro{MAR}{Medication Administration Records}
\acro{CBC}{Complete Blood Count}
\acro{ESR}{Erythrocyte Sedimentation Rate}
\acro{EMRs}{Electronic Medical Records}
\acro{PROs}{Patient Reported Outcomes}
\acro{CNNs}{Convolutional Neural Networks}
\acro{PCA}{Principal Component Analysis}
\acro{t-SNE}{t-distributed Stochastic Neighbor Embedding}
\acro{RL}{Reinforcement Learning}
\acro{IoT}{Internet of Things}
\acro{DApps}{Decentralized Applications}
\acro{P2P}{Peer-to-Peer}
\acro{PoW}{Proof of Work}
\acro{PoS}{Proof of Stake}
\acro{IBC}{Inter-Blockchain Communication}
\acro{DPoS}{Delegated Proof of Stake}
\acro{BFT-based consensus}{Byzantine Fault Tolerant-based consensus}
\acro{BFT}{Byzantine Fault Tolerance}
\acro{pBFT}{Practical Byzantine Fault Tolerance}
\acro{PoC}{Proof of Capacity}
\acro{PoST}{Proof of Space and Time}
\acro{DAG}{Direct Acyclic Graph Tangle}
\acro{PoB}{Proof of Burn}
\acro{PoA}{Proof of Authority}
\acro{DeFi}{Decentralized Finance}
\acro{IoB}{Internet of Blockchains}
\acro{MNIST}{Modified National Institute of Standards and Technology}
\acro{IoMT}{Internet of Medical Things}
\acro{GANs}{Generative Adversarial Networks}
\acro{CPS}{Cyber-Physical Systems}
\acro{HAM10000}{Human Against Machine with 10000 training samples}
\acro{FL-BETS}{FL-based BC-enabled task scheduling}
\acro{ML}{Machine Learning}
